Dynamic Interference Prediction for In-X 6G Sub-networks

The sixth generation (6G) industrial Sub-networks (SNs) face several challenges in meeting extreme latency and reliability requirements in the order of 0.1-1 ms and 99.999 -to-99.99999 percentile, respectively. Interference management (IM) plays an integral role in addressing these requirements, especially in ultra-dense SN environments with rapidly varying interference induced by channel characteristics, mobility, and resource limitations. In general, IM can be achieved using resource allocation and \textit{accurate} Link adaptation (LA). In this work, we focus on the latter, where we first model interference at SN devices using the spatially consistent 3GPP channel model. Following this, we present a discrete-time dynamic state space model (DSSM) at a SN access point (AP), where interference power values (IPVs) are modeled as latent variables incorporating underlying modeling errors as well as transmission/protocol delays. Necessary approximations are then presented to simplify the DSSM and to efficiently employ the extended Kalman filter (EKF) for interference prediction. Unlike baseline methods, our proposed approach predicts IPVs solely based on the channel quality indicator (CQI) reports available at the SN AP at every transmission time interval (TTI). Numerical results demonstrate that our proposed approach clearly outperforms the conventional baseline. Furthermore, we also show that despite predicting with limited information, our proposed approach consistently achieves a comparable performance w.r.t the off-the-shelf supervised learning based baseline.

==> extras/extras.tex <==
In this work, we focus on an \gls{In-F} \gls{SN} scenario with latency and reliability requirements in the order of approximately $0.1ms$ and $6-9$ nines respectively. 

into the larger macro-network \pramesh{6G Network?}

Inter-(and intra-)\gls{SN} interference arises as a natural phenomenon due to ultra-dense deployments, rapid variations in \gls{HRLLC} traffic patterns and fading effects due to the underlying wireless channel. Therefore, \gls{IM} plays an important aspect in realizing the \glspl{SN}.

The \gls{SN} controller is assumed to be positioned at the center whose positions are denoted as $\mathbf{P}= [\mathbf{p}_{n_1},\dotsc, \mathbf{p}_{n_{N}}]$. Assume that

Further details can be found in \cite{gautam2023co}.

where a sub-band is assumed to be allocated for one specific \gls{SN}.

We assume that by proper allocation of the time unit, there is no intra-\gls{SN} interference . We assume the number of sub-bands . Therefore, multiple \glspl{SN} will interfere while operating on a single sub-band.

Consequentially, there exists dynamic inter-\gls{SN} interference due to the sub-band sharing by more than one moving \gls{SN}. 

We characterize the \gls{SN} interference for the Uplink scenario ensuing between a \gls{SN} controller, however similar analysis can be applied .

 and $\mathcal{\hat{N}}\setminus\{n_{q}\}$ \glspl{SN} interfering with $n_q$th \gls{SN}.

    \item . Here, \gls{CQI} values are quantized information reported by associated \glspl{UE}~\cite{3gpp2018physical}; \gls{MCS} selection by repeated transmissions and ACK/NACK feedback adjustments~\cite{pocovi2018joint,brighente2020interference}

% The overall \gls{LA} is summarized as follows in algorithm \cref{algo:proposed_algo}:
% \begin{algorithm}
% \caption{Link Adaptation with Interference Prediction for In-X Subnetwork}
% \label{algo:proposed_algo}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Target \gls{BLER} $\varepsilon_{\text{target}}$, estimated CSI $\hat{S}_{n_q}$, Received \gls{CQI} $y_{n_{q}}$ at \gls{SN} controller
% \State \hspace{\algorithmicindent} List of achieved \gls{BLER} $\boldsymbol{\varepsilon}$
% \For{$i = 1, \dots$}
% \State Predict $\hat{I}_{n_{q}}(t)$ using \gls{EKF}/Moving-Average/\gls{LSTM}
% \State Perform SINR adjustment and calculate $\hat{\gamma}_{n_{q}}(t)$
% \State Select \gls{MCS} from look-up table with: 
% \Statex \hspace{\algorithmicindent} \begin{align*}
% \max_{m(t)} R(m(t)) \\ \text{s.t. } \varepsilon(t) \leq \varepsilon_{\text{target}}
% \end{align*}
% \State Store achieved \gls{BLER} $\boldsymbol{\varepsilon} \leftarrow \varepsilon (t)$
% \EndFor
% \end{algorithmic}
% \end{algorithm}

This is followed by an \gls{OLLA} step, which assists \gls{MCS} selection by repeated transmissions and ACK/NACK feedback adjustments~\cite{brighente2020interference}.

% The thermal noise $w$ is calculated as $w= JTB \cdot 10^{\dfrac{NF}{10}}$, where $J$ represents the Boltzmann constant, $T$ denotes the temperature in Kelvin, $B$ indicates the bandwidth in Hertz, and $NF$ signifies the Noise Figure in decibels (dB).

%The schematic of the \gls{LA} is illustrated in \cref{Fig:la_schemetics}. The \gls{SN} controller transmits \gls{CSI-RS} to the \gls{SA} pair, which in turn sends \gls{CQI} back to the \gls{SN} controller. Based on the received \gls{CQI}, the channel quality, i.e., \gls{SINR}, is predicted. Following the adjustment of the predicted \gls{SINR}, an appropriate MCS is selected while considering a use case specific target \gls{BLER}. The \gls{MCS} comprises the \gls{MO} and the \gls{CR}. When the link between the \gls{SA} pair and \gls{SN} controller exhibits good quality, allowing for high throughput with a certain error probability, the \gls{SN} controller opts for higher \gls{MO} and \gls{CR}. Conversely, if the link quality is poor, the \gls{SN} controller selects smaller \gls{MO} and \gls{CR} to maintain a similar error probability, albeit at the expense of throughput. Industrial factory \glspl{SN} aim for extremely low latency, measured in fractions of milliseconds, with packets expected to transmit only once. Reliability targets are set to achieve a defined target \gls{BLER} within a single transmission attempt. Thus, the \gls{LA} strategy in this work is assumed to pick an \gls{MCS} that can meet a certain target \gls{BLER} for the packet according to the estimated channel. By this configuration, we can select $\mu(t)$  among a list of \glspl{MCS} based on the channel quality as follows:

%Once we calculate the achieved \gls{BLER} by utilizing the selected \gls{MCS}, we evaluate the \gls{ECDF} of the proposed and baseline methods as performance metrics to conclude the efficacy of proposed state-space modeling and baseline methods. 

An \gls{SA}-pair prepares the \gls{CQI} report based on the \gls{SNR} estimate obtained from the reference signals.

However,  Secondly, the \gls{CQI} report prepared by an \gls{SA}-pair is based on \gls{EESM} mechanisms, which map \gls{SNR} estimates to the effective \gls{SNR} followed by a quantization step, which is based on predefined lookup tables. Both these          

\ravi{Self: quantization error, protocol and transmission delays + overhead of transmitting interference information from SA pairs to the controller and hence the need for interference prediction + DSS modeling since interference is a latent variable of CQI report.}.  

is usually performed with outdated \gls{CQI} information, which is caused due to inherent protocol overhead and transmission delays. In a rapidly varying interference environments projected by the \gls{SN} devices, the outdated \gls{CQI} information can heavily impact the \gls{MCS} selection. thus also negatively impacting the latency and reliability aspects. We are interested in proactive interference estimation, i.e., prediction at the \gls{SN} controller at time $t$.

The position of the \gls{SA} pair $m$ of the $n$ \gls{SN} is therefore $\boldsymbol{\phi}_{n_{q}m_{a}}= \mathbf{p}_{n_q} + \boldsymbol{\xi}_{n_{q}m_{a}}$, where $\boldsymbol{\xi}_{n_{q}m_{a}}$ is the position of \gls{SA} pair.

 
% Let $\mathscr{B}\left(\mathbf{p}_{n},r\right)$ denote a disc with radius $r$ centered at position $\mathbf{p}_{n}:=(x_{n},y_{n})$, thereby jointly defining the area occupied by the $n^{\text{th}}$ \gls{SN}. We consider that the \gls{SA} pairs are distributed according to a binomial point process whose p.d.f is given by $(\pi r^{2})^{-1}$ in a disc of radius $r$, i.e., in $\mathscr{B}(\pmb{0},r)$. 

\subsection{Channel and Interference Modeling}
\label{sec:interferencemodeling}

\footnote{Current modeling and analysis can be applied to uplink with minor modifications.}

, with $r$ being the radius of the disc encircled around a controller

We generate the \gls{CQI} $y_{n}(t)$ based on the \gls{SINR}, computed using $g_{2}(g_{1}(\gamma_{n}(t)))$, where 

while transmitting a packet from \gls{SN} controller to \gls{SA} pair for downlink and \gls{SA} pair to \gls{SN} controller.

Assuming unit energy for the transmitted baseband signal, 

% \begin{multline}
% \label{eq:laprob}
% \phi_{m_a}^*(t) = \sup\{R(\phi_{m_a}(t)) | \varepsilon(\phi_{m_a}(t)) \leq \Bar{\varepsilon}, \phi_{m_a}(t) \in \Phi \},
% \end{multline}

%$\phi_{m_a}^*(t)$



In this section, we relate the State space modeling of \gls{SN} interference and predict the interference using \gls{EKF} for the aforementioned problem description.
\subsection{State Space Modeling of \gls{SN} Interference}
We consider the estimation of the \gls{CQI} at the \gls{SA} pair to occur at time $t-1$. The estimated \gls{CQI} will be sent to the \gls{SN} controller at the beginning of time $t$.  The interference prediction problem by considering interference as a hidden state derived from the received \gls{CSI}, i.e., \gls{CQI} can be formulated as:
% \begin{align}
%     I_{n}(t) &:= f(\mathbf{I}_{n}(t-1),\nu(t)), & \nu(t) &\sim \mathcal{N}(0,\Omega) \label{eq:1} \\
%     y_{n}(t) &:= \tilde{g}(I_{n}(t),w(t)), & w(t) &\sim \mathcal{N}(0,R) \label{eq:2}
% \end{align}

\begin{align}
    &I_{n}(t) := f(I_{n}(t-1))+\nu(t), & \nu(t) &\sim \mathcal{N}(0,\sigma_f) \label{eq:dssma} \\
    &Y_{(n,m)}(t) := g(I_{n}(t))+u(t), & u(t) &\sim  \mathcal{N}(0,\sigma_g). \label{eq:dssmb}
\end{align}

\subsection{Extended Kalman Filter-based Predictor}

In this paper, we aim to predict interference at the \gls{SN} controller utilizing only \gls{CQI} data. In every \gls{TTI} $t$, \gls{EKF} predicts  $\hat{I}_{n}(t)$ utilizing previous predictions $\hat{\textbf{I}}_{n}(t-1)$ and new observed \gls{CQI} $Y_{n}(t)$. The proposed method operates through a simple two-step process: prediction and update \cite{kay1993fundamentals}. In the prediction step, the current a priori statistical moments of $\mathbf{I}_{n}$ are computed utilizing previous a posteriori prediction together with knowledge of the state evolution matrix $\mathbf{F}$ as:
\begin{equation}\label{eq:ekf1}
\begin{aligned}
    \hat{I}_{n}(t|t-1) &= \mathbf{F} \cdot \mathbf{\hat{I}}_{n}(t-1), \\
    {\Sigma }(t \big| t-1 ) &= \mathbf{F} \cdot {\Sigma }(t-1 \big| t-1)\cdot \mathbf{F}^\top +{\sigma_{f}},
\end{aligned}
\end{equation}

and the moments of the observed \gls{CQI} $y_{n}(t)$ based on the knowledge $G(t)$ as 
\begin{equation}\label{eq:ekf2}
\begin{aligned}
    \hat{Y}_{n}(t|t-1) &= G(t) \cdot \hat{I}_{n}(t|t-1), \\
    {S}(t \big| t-1 ) &= {{G(t)}}\cdot {\Sigma }(t \big| t-1) \cdot {{G(t)}}^\top +\sigma_{g}.
\end{aligned}
\end{equation}
In update step, we utilize a priori moments from \cref{eq:ekf1} and \cref{eq:ekf2} to calculate a posteriori state moments as follows:
\begin{equation}
\begin{aligned}
    \hat{I}_{n} (t | t) &= \hat{I}_{n}(t | t-1)+{\mathcal{K}}(t)\cdot {\Delta} {Y}_{n}(t), \\
    \Sigma(t | t) &= (1-\mathcal{K}(t)\cdot  G(t))\cdot {\Sigma }(t \big| t-1),
\end{aligned}
\end{equation}

where $\mathcal{K}(t)$ is the Kalman Gain and it is given as:
\begin{align}
    &\mathcal{K}(t)={{\Sigma }}(t \big| t-1 )\cdot  {G}(t) \cdot { {S}}^{-1}(t \big| t-1 ).
\end{align}
The term \( \Delta Y_{n}(t) = Y_{n}(t) - \hat{Y}_{n}(t | t-1) \) represents the innovation, which adjusts the predictions to be more accurate by combining the latest observed CQI in state space modeling. Leveraging the calculated Kalman Gain \( \mathcal{K}(t) \), the EKF adjusts the residual to refine the state estimate \( \hat{I}_{n} (t | t) \) and its uncertainty \( \Sigma(t | t) \), effectively integrating the predictive model with CQI. Through this iterative mechanism, the EKF persistently refines its state estimates, thereby ensuring interference prediction with minimal predictor error over time. This iterative process of predicting interference and subsequently refining it based on newly observed CQI enables the EKF to accurately capture the dynamic nature of interference over time.

% \section{Link Adaptation Adjustments for \glspl{SN}} \label{sec.la}

% The schematic of the \gls{LA} is illustrated in \cref{Fig:la_schemetics}. The \gls{SN} controller transmits \gls{CSI-RS} to the \gls{SA} pair, which in turn sends \gls{CQI} back to the \gls{SN} controller. Based on the received \gls{CQI}, the channel quality, i.e., \gls{SINR}, is predicted as mentioned in the previous section.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\linewidth]{images/block_diagram_1.png}
%     %\includegraphics[width=0.99\linewidth]{images/block_diagram_2.png}
%     \caption{Proposed Link Adaptation for In-X \gls{SN}}
%     \label{Fig:la_schemetics}
% \end{figure}
% Following the adjustment of the predicted \gls{SINR}, an appropriate MCS is selected while considering a use case specific target \gls{BLER}. The \gls{MCS} comprises the \gls{MO} and the \gls{CR}. When the link between the \gls{SA} pair and \gls{SN} controller exhibits good quality, allowing for high throughput with a certain error probability, the \gls{SN} controller opts for higher \gls{MO} and \gls{CR}. Conversely, if the link quality is poor, the \gls{SN} controller selects smaller \gls{MO} and \gls{CR} to maintain a similar error probability, albeit at the expense of throughput. Industrial factory \glspl{SN} aim for extremely low latency, measured in fractions of milliseconds, with packets expected to transmit only once. Reliability targets are set to achieve a defined target \gls{BLER} within a single transmission attempt. Thus, the \gls{LA} strategy in this work is assumed to pick an \gls{MCS} that can meet a certain target \gls{BLER} for the packet according to the predicted channel. We evaluate the performance of proposed predictor with baseline predictor in next section.

% In this work, we aim to predict interference at the \gls{SN} controller using only \gls{CQI} data. To predict interference, denoted as $I_{n}(t)$, from observed \gls{CQI} $y_{n}(t)$, we employ an Extended Kalman filter. First of all, we linearize the nonlinear relationship of \cref{eq:1}.  Interfering links, expected to have a lower \gls{LOS} probability due to spatial distance between interferers and the receiver, indirectly favor interference following a Rayleigh distribution. This paper exclusively focuses on the Bessel function related to Rayleigh fading, leaving the dynamics between Rice and Rayleigh fading as an open topic for further investigation. By considering a correlation matching criterion, the coefficient for linearization with predicted interference for previous \gls{TTI} $\hat{I}_{n}(t-1)$ can be related by $\alpha_{b} = J_{0}(w_{d} \cdot \tau)$ \cite{ghandour2012use}. The linearized model is considered as $\hat{I}_{{n}}(t)= \alpha_{b} \hat{I}_{{n}}(t-2) + (1- \alpha_{b}) \hat{I}_{{n}}(t-1)$. Moreover, for linearizing \cref{eq:2}, we consider that the received \gls{CQI} is a wideband and dequantized value from the \gls{CQI}. The estimated \gls{SINR} with quantization error can be linked with interference by \cref{eq:sinr}. We use the Jacobian to linearize this model as 
% \begin{align}
%     G(t): = \frac{\partial {\gamma}_{n}(t)}{\partial \hat{I}_{n}(t)},
% \end{align}
% which simplifies the impact of changes in interference in \gls{CQI}. 


% Moreover, it is observed that small-scale fading predominantly influences the channel correlation, which can be described using the zeroth-order modified Bessel function \(J_{0}(w_{d} \cdot \tau)\), where $w_{d}$ is Doppler spread and $\tau$ is the duration of \gls{TTI} for Rayleigh fading \cite{xiao2006novel}. In the case of Rice fading, the envelope of the \gls{PDF} can be represented by the zeroth-order modified Bessel function \(J_{0}(2 z \sqrt{K(1+K)})\), where $K$  and $z$ are rice factor and fading envelope respectively \cite{xiao2006novel}.

% As we consider dequantized data as input, we need to reflect quantization, compression and reconstruction error in terms of variance $R$. We have considered that the variance $R$ arises from the combination of quantization error, with variance $\mathcal{N}(0,\sigma_{q}^{2})$, and process noise, with variance $\mathcal{N}(0,\sigma_{g}^{2})$. We consider the variance associated with quantization error as $\mathcal{N}(0,\sigma_{q}^{2})$ for uniform quantization of minimum and maximum \gls{SINR}. As the quantization method may vary depending on the use case specification, the variance can be replaced by the respective quantization error variance determined by the selected quantization technique. After linearizing the model, we proceed with the prediction using the Kalman filter \cite{kay1993fundamentals}.



% The overall interference prediction can be summarized in the following algorithm:

% \begin{algorithm}
% \caption{Extended Kalman Filter for Interference Prediction \cite{kay1993fundamentals}}
% \label{algo:proposed_algo}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Received CQI $y_{n}(t)$ at SN controller
% \For{$i = 1, \dots$}
% \State Prediction:  $\hat{I}_{n}(t| t-1 ) = \alpha_{b}\cdot \hat{I}_{n}(t-1 | t-1 )+ (1-\alpha_{b})\cdot \hat{I}_{n}(t-1 | t-2 )$
% \State Minimum Prediction MSE: ${\Sigma }(t \big| t-1 ) = {\alpha_{b}}^2 \cdot {\Sigma }(t-1 \big| t-1) +{Q}$
% \State Measurement residual: ${S}(t \big| t-1 ) = {{G(t)}}\cdot {\Sigma }(t \big| t-1) \cdot {{G(t)}}^\top +R$
% \State Kalman Gain:  $\mathcal{K}(t)=\dfrac{{{\Sigma }}(t \big| t-1 )\cdot { {G}}}{ { {S}}^{-1}(t \big| t-1 )}$
% \State Update State estimate: $\Delta  {y}_{n}(t)= {y}_{n}(t)-\hat{ {y}}_{n}(t \big| t-1 )$
% \State  Correction: $\hat{I}_{n} (t | t)= \hat{I}_{n}(t | t-1)+{\mathcal{K}}(t)\cdot {\Delta} {y}_{n}(t)$
% \State Minimum MSE: $\Sigma(t | t) = (1-\mathcal{K}(t)\cdot  G(t))\cdot {\Sigma }(t \big| t-1)$
% \EndFor
% \end{algorithmic}
% \end{algorithm}
% The proposed method operates through a simple two-step process: prediction and correction. Initially, it uses current information to predict the future state of the system $\hat{I}_{n}(t| t-1 )$ and its uncertainty $\boldsymbol{\Sigma }(t | t-1 )$. Then, when new data comes in, it measures the difference $\hat{y}_{n}(t | t-1 )$ between what was predicted and what actually happened. This process helps adjust the predictions to be more accurate, combining what was expected with the latest measurements. Leveraging the calculated Kalman Gain $\mathcal{K}(t)$, the \gls{EKF} adjusts this residual to refine the state estimate $\hat{I}_{n} (t | t)$ and its uncertainty $\Sigma(t | t)$, effectively integrating the predictive model with incoming data. This iterative mechanism, which adeptly minimizes estimation errors through a dynamic equilibrium between model forecasts and measurement accuracy, establishes the \gls{EKF} as an essential tool for achieving optimal state estimation in real-time and dynamic systems. Through the continuous application of these steps, the \gls{EKF} persistently refines its state estimates, thereby ensuring high precision in the system's state approximation over time. This ongoing process of predicting interference and subsequently refining based on newly observed \gls{CQI} enables the \gls{EKF} to accurately capture the dynamic nature of interference over time.

From a network deployment perspective, a typical  (collectively referred to as \glspl{UE} in this work).

In this work, we propose a proactive interference estimation, i.e., a prediction technique to address these challenges. We model \gls{SN} interference and propose an online-unsupervised \gls{EKF} for interference prediction.
% To overcome these challenges, in this work, we propose a proactive interference prediction mechanism  address these challenges, in \gls{IPV} this work, we model the \gls{SN} interference and propose an online-unsupervised \gls{EKF} for interference prediction.
The proposed method predicts interference from \gls{CQI}, which is available data at \gls{SN} controller. Interference, considered a latent variable of \gls{CQI}, is the primary cause of non-linear dynamics and high variation in CQI, directly limiting the capability to achieve aforementioned extreme heterogeneous requirements. The proposed state-space model can accommodate noise associated with measurement, quantization, and other factors as well. Moreover, this proposed method does not necessarily require a label, i.e., the interference power value at the \gls{SN} controller, thereby reducing communication costs to transfer those \glspl{CSI} to the \gls{SN} controller, unlike \cite{gautam2023co}.

This is in contrast to the existing literature where interference prediction/estimation is performed as a \gls{UE}-side operation


% In this paper, we refer to them as \gls{AP} and \gls{UE} to preserve consistency.   


% A typical \gls{SN} comprises of an \gls{AP} and several \glspl{UE} either connected to the controller or communicating among themselves. The \gls{SN} devices are envisioned to operate in short-ranges with \gls{HRLLC} traffic requirements. More information on common \gls{SN} use-cases and deployment scenarios can be found in~\cite{berardinelli2021extreme}.


% The \gls{6G} industrial \glspl{SN} face several challenges in meeting extreme latency and reliability requirements ranging in the order of $0.1ms$ and $6-to-9$ nines, respectively. \gls{IM} plays a key role in addressing these requirements, especially in ultra-dense \gls{SN} environments with rapidly varying interference caused due to mobility, resource limitations and channel characteristics. \gls{IM} for \glspl{SN} typically involve meticulous resource allocation mechanisms and accurate \gls{LA} schemes. In this work, we focus on \gls{IM} using \gls{LA} improvements, where we first characterize interference of \gls{SN} devices using spatially consistent 3GPP channel model and the assumed traffic pattern. Following this, we propose a low-complexity \gls{EKF}-based interference prediction algorithm operating at every \gls{TTI}. Unlike baseline supervised approaches, the \gls{EKF} algorithm predicts the interference for the next \gls{TTI} solely based on the \gls{CQI} information available at a \gls{SN} controller. Finally, we evaluate the performance of our proposed method and compare it against the baseline methods.

%In view of the above-mentioned challenges, in this work, we model and propose an interference prediction mechanism at an \gls{AP} which assists the \gls{LA} scheme in achieving the desired reliability requirements. Prior to highlighting the contributions of this work, we first discuss some relevant research work on interference prediction for \gls{LA} improvements.

% Our proposed method considers the prediction of interference is performed at the \gls{SN} controller and the available data is  CQI only. The CQI is generated uniformly quantized from estimate  \gls{SINR} into $5$ bit with 32 \gls{MCS} as specified in \cite{3gpp2018physical}. We assume that \glspl{CQI} is only the available data with \gls{SN} controller, which carries the information about the dynamics of channel statics together with mobility and short packet traffic.  We propose the technique to predict interference at the next transmit time interval \gls{TTI} from the currently observed CQI. Learning these dynamics helps to mitigate the effect of CQI expiry and is anticipated to help achieve effective MCS selection \cite{ramezani2021cqi}. Hence, we propose an extended Kalman filter for interference prediction by observing CQI at the \gls{SN} controller which works as unsupervised learning fashion. 



\textit{\textbf{Contribution 1:}}  The proposed state-space modeling employing the \gls{EKF} predicts interference in an online, unsupervised manner by leveraging accessible CSI data at the \gls{SN} controller, specifically the \gls{CQI}. Furthermore, this state-space prediction framework accounts for quantization, compression, reconstruction errors, and process noise. It also integrates the correlation coefficient of small-scale fading to bolster predictor performance. This method doesn't need the interference power value, i.e., a label at the \gls{SN} controller, which makes the cost associated with transferring that interference data redundant.

\textit{\textbf{Contribution 2:}} The predicted interference has been utilized for link adaptation purposes to select the optimal \gls{MCS}, ensuring the target \gls{BLER}, which has been considered as a reliability measure. The efficacy of the proposed method is evaluated using a spatially consistent \gls{3GPP} channel model for indoor factory scenarios. Moreover, 

Moreover, unlike baseline \gls{LA} schemes, this approach does not require explicit feedback from associated \glspl{UE} thus being well suited for \gls{HRLLC} traffic.



In this work, the inter-dependencies between \glspl{IPV} and the available \gls{CQI} reports as a \gls{DSSM} at an \gls{AP}, we consider the following aspects:
\begin{enumerate}[label=(\alph*)]
    \item Firstly, .
    \item As mentioned in section~\ref{sec:introduction}, the  Thus, \glspl{IPV} can be modeled as the hidden/latent state of the \gls{CQI} report.
    \item One can recall from section~\ref{sec:systemmodel} that , all the 
\end{enumerate}

 The \gls{DSSM} in~\eqref{eq:dssm} is non-linear in nature due to the observation function, $G(.)$, which is characterized by~\eqref{eq:sinr}

 % The latent variable interference is related to the received \gls{CQI} by the function $g(\cdot)$ as \cref{eq:dssma}. 

 Hence, the \textit{modified \gls{DSSM}} with vector notation for state evolution of \glspl{IPV} over \gls{TTI} and the observation model transformation can be expressed as:
\begin{align}\label{eq:approx_state}
    f(\hat{\mathbf{I}}_{n}(t-1)) \approx  \mathbf{F} \cdot \hat{\mathbf{I}}_{n}(t-1) , \  g(\hat{I}_{n}(t)) \approx G(t) \cdot \hat{I}_{n}(t).
\end{align}

\begin{equation}\label{eq:ekf1}
\begin{aligned}
    \hat{I}_{n}(t|t-1) &= \mathbf{F} \cdot \mathbf{\hat{I}}_{n}(t-1), \\
    {\Sigma }(t \big| t-1 ) &= \mathbf{F} \cdot {\Sigma }(t-1 \big| t-1)\cdot \mathbf{F}^\top +{\sigma_{f}},
\end{aligned}
\end{equation}

and the moments of the observed \gls{CQI} $y_{n}(t)$ based on the knowledge $G(t)$ as 
\begin{equation}\label{eq:ekf2}
\begin{aligned}
    \hat{Y}_{n}(t|t-1) &= G(t) \cdot \hat{I}_{n}(t|t-1), \\
    {S}(t \big| t-1 ) &= {{G(t)}}\cdot {\Sigma }(t \big| t-1) \cdot {{G(t)}}^\top +\sigma_{g}.
\end{aligned}
\end{equation}
In update step, we utilize a priori moments from \cref{eq:ekf1} and \cref{eq:ekf2} to calculate a posteriori state moments as follows:
\begin{equation}
\begin{aligned}
    \hat{I}_{n} (t | t) &= \hat{I}_{n}(t | t-1)+{\mathcal{K}}(t)\cdot {\Delta} {Y}_{n}(t), \\
    \Sigma(t | t) &= (1-\mathcal{K}(t)\cdot  G(t))\cdot {\Sigma }(t \big| t-1),
\end{aligned}
\end{equation}

where $\mathcal{K}(t)$ is the Kalman Gain and it is given as:
\begin{align}
    &\mathcal{K}(t)={{\Sigma }}(t \big| t-1 )\cdot  {G}(t) \cdot { {S}}^{-1}(t \big| t-1 ).
\end{align}
The term \( \Delta Y_{n}(t) = Y_{n}(t) - \hat{Y}_{n}(t | t-1) \) represents the innovation, which adjusts the predictions to be more accurate by combining the latest observed CQI in \gls{DSSM} modeling. Leveraging the calculated Kalman Gain \( \mathcal{K}(t) \), the EKF adjusts the residual to refine the state estimate \( \hat{I}_{n} (t | t) \) and its uncertainty \( \Sigma(t | t) \), effectively integrating the predictive model with CQI. Through this iterative mechanism, the EKF persistently refines its state estimates, thereby ensuring interference prediction based on newly observed CQI with minimal predictor error over time. 
% This iterative process of predicting interference and subsequently refining it based on newly observed CQI enables the EKF to accurately capture the dynamic nature of interference over time.

% An important point to notice in~\eqref{eq:dssmb} is that we consider the \gls{CQI} of $Y_{(n,m)}(t)$ of the $m^{\text{th}}$ \gls{SA}-pair  We consider $\nu(t)$ and $u(t)$ as Gaussian noise with known variance $\sigma_{f}$ and $\sigma_{g}$ respectively. The variance $\sigma_{f}$ represents the combination of the noise variance related to the scheduling of neighboring SN and interference modeling noise. Whereas, $\sigma_{g}$ represents the quantization and dequantization noise while mapping \gls{eSNR} to \gls{CQI}. Here, the function $g = g_{1} \circ g_{2}$ is the function composition of \gls{eSNR} mapping using \gls{ESM} after \gls{SINR} quantization.
% % The dynamics of interference referring to the previous \gls{TTI} is defined by function $f(.)$. 
% The variance of $g$ arises from the product of two Gaussian distributions, yielding a Gaussian distribution with a variance \cite{bromiley2003products} as 
% \begin{align}
%  \sigma_{g} = \frac{\sigma_{g_{1}}^{2} \cdot \sigma_{g_{2}}^{2}}{\sigma_{g_{1}}^{2} + \sigma_{g_{2}}^{2}},
% \end{align}
% where $\sigma_{g_{1}}$ and $\sigma_{g_{2}}$ are variance associated with $g_1$ and $g_2$. In this work, we consider the state evolution of \glspl{IPV} and the measurement model transformation to be linear and expressed as follows:
% \begin{align}
%     f(\mathbf{I}_{n}(t-1)) \approx  \mathbf{F} \cdot \mathbf{I}_{n}(t-1) , \  g(I_{n}(t)) \approx G(t) \cdot I_{n}(t).
% \end{align}

% We consider the state evolution in \cref{eq:dssma} to be due to small-scale fading as the primary source of correlation, and thus, we have incorporated its approximate solution accordingly. The correlation due to small-scale fading can be approximated by zeroth-order modified Bessel function $B_{0}(w_{d} \cdot \tau)$, where $w_{d}$ is Doppler spread and $\tau$ is the duration of \gls{TTI} for Rayleigh fading \cite{xiao2006novel}.
% % In the case of Rice fading, the envelope of the \gls{PDF} can be represented by the zeroth-order modified Bessel function $B_{0}(2 z \sqrt{K(1+K)})$, where $K$  and $z$ are rice factor and fading envelope respectively \cite{xiao2006novel}. 
% In this work, we focus on the Bessel function related to Rayleigh fading, leaving the dynamics between Rice and Rayleigh fading as an open topic for further investigation. By adopting a correlation matching criterion \cite{ghandour2012use}, the state evolution vector for predicted interference at time $t$ utilizing previously predicted interferences at $t-1$ and $t-2$ \glspl{TTI}, is represented as  $\mathbf{F} =  [\alpha_{b},1- \alpha_{b}]$, where $\alpha_{b} = B_{0}(w_{d} \cdot \tau)$. The transformation can be expressed as  
% \begin{align}
%     \hat{I}_{{n}}(t) \approx \alpha_{b} \hat{I}_{{n}}(t-2) + (1- \alpha_{b}) \hat{I}_{{n}}(t-1) : =  \textbf{F} \cdot \mathbf{\hat{I}}_{n}(t-1).
% \end{align}
% where $\mathbf{\hat{I}}_{n}(t-1) = [\hat{I}_{{n}}(t-1),\hat{I}_{{n}}(t-2)]^\top$ is previously predicted \glspl{IPV}. The latent variable interference is related to the received \gls{CQI}, which is a quantized value resulting from \gls{SINR} mapping via \cref{eq:sinr}. Considering wideband \gls{CQI}, and the function $g(\cdot)$ being differentiable in a time-dependent manner, we express this using partial derivatives through the Jacobian as:
% \begin{align}
%     G(t): = J_{I_{n}}(g(t)),
% \end{align}
% thus simplifying the evaluation of interference-induced changes in \gls{CQI}.

% We show that the proposed method, performed solely based on the available \gls{CQI} reports as observations and without any explicit feedback/labels, can achieve a comparable performance w.r.t the Genie \gls{LA} baseline.

Unlike this work, \cite{gautam2023co} assumes that the noise-free \gls{IPV} is known at the \gls{AP}.

 The data is restructured with a sliding window $\Omega_{W}$ and a step size of $\Omega_{p}$. The task is to predict the interference of the $n$th \gls{SN} at time $t$ by utilizing the IP vector  for a trained model of the respective \gls{SA} pair's \glspl{IPV} as 
\begin{align} \label{eq:onetoone}
\hat{I}_{n}(t)= f_{\textbf{w}}(\tilde{\mathbf{I}}_{n}(t-1)^{T}),
\end{align}
where $\textbf{w}$ is trained \gls{LSTM} model parameter. 

We assume that $16$ uniformly distributed \glspl{SN} are deployed in a confined area of $20 \times 20 \, \text{m}^2$, each moving at a constant velocity of $2 \, \text{m/s}$ in a random direction with $\theta$ drawn from a uniform distribution between $0$ and $2 \pi$. We consider a single \gls{UE} distributed with a binomial point process whose p.d.f is given by $(\pi r^{2})^{-1}$ in a disc of radius $r =2$.  The \glspl{SN} follow the \gls{RDMM}. Due to dynamic mobility of  \glspl{SN}, there is a possibility that receivers or potential interferers may be in either \gls{LOS} or \gls{NLOS} conditions. We consider a spatially consistent \gls{3GPP} channel model related to the \gls{InF-DL}, which is suitable for our considered use case.
% The proposed interference model accounts for the \gls{LOS} probability as those \glspl{SN} move dynamically, which has the ability to adapt to the possibility of change in \gls{LOS} and \gls{NLOS} as well. The respective parameters related to free space path loss and shadowing for \gls{LOS} and \gls{NLOS} have been used from \cite{3gpp2018study}.
The additional parameters associated with the channel are specified in \cref{table:2}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\linewidth]{images/plot.eps}
%     \caption{Prediction of interference for a fixed time step~(test data)}
%     \label{fig:predictiontrajectory}
% \end{figure}

To ensure a fair comparison between the proposed method and \gls{LSTM}, we utilized $20,000$ predicted interference power values, selected from the unseen test data comprising $20\%$ of the total $100,000$ samples, for evaluation against the \gls{LSTM}-based predictor.

as an online and unsupervised learning method, the \gls{EKF} leads to a prediction error of $1.31$ dB at the $50$th percentile as

Furthermore, it is necessary to analyze the discrepancy in the performance of those predictors for \gls{IM} in terms of achievable \gls{BLER} by selecting \gls{MCS} based on predicted interference. 

% We utilize the predicted interference to adjust the \gls{SINR} for the next \gls{TTI} considering $S_{(n,m)}$ is perfectly known due to short-range communication, along with the fixed position of the \gls{SN} controller and \gls{SA} pair. 

More precisely, this exercise throws light on the importance of  appropriate \gls{MCS} selection to extreme reliability requirements in the \gls{DL}.

% Once the \gls{MCS} is selected from the predicted interference, \gls{BLER} is retrieved from the \gls{MCS} look-up table corresponding to the predicted \gls{SINR}, allowing us to assess the difference between the targeted and observed \gls{BLER}, reflecting the comparison between the actual and predicted \gls{SINR}. 

The results in \cref{fig:bler_ecdf} illustrate that based on the selected \gls{MCS}, the

Both \gls{EKF} and \gls{LSTM} effectively predict interference and achieve \glspl{BLER} comparable to those of Genie \gls{LA}. In contrast, the moving average predictor results significant deviations as compared to Genie \gls{LA}. Notably, Genie \gls{LA} tends to slightly outperform the target \gls{BLER} due to the limited number of \glspl{MCS} available as shown in  Fig.~1 of \cite{alonzo2020urllc}. 

 on \glspl{SN},

 on \glspl{SN},

 \textcolor{blue}{Furthermore, 6G is envisioned to provide technological capability by providing \gls{HRLLC} as a sixth pillar for use cases with extreme requirements, such as $0.1-1$ ms latency and $99.999-99.99999$ percentile reliability~\cite{recommendation2023framework}.}


==> extras/proposedpredictor_dump.tex <==
\section{State Space Modeling of \gls{SN} Interference}
We consider the estimation of the \gls{CQI} at the \gls{SA} pair to occur at time $t-1$. The estimated \gls{CQI} will be sent to the \gls{SN} controller at the beginning of time $t$.  The interference prediction problem by considering interference as a hidden state from received \gls{CSI}, i.e., \gls{CQI} can be formulated as:
\begin{align}
    I_{n_{q}}(t) &:= f(\mathbf{I}_{n_{q}}(t-1),\nu(t)), & \nu(t) &\sim \mathcal{N}(0,\Omega) \label{eq:1} \\
    y_{n_{q}}(t) &:= \tilde{g}(I_{n_{q}}(t),w(t)), & w(t) &\sim \mathcal{N}(0,R) \label{eq:2}
\end{align}
Here, $y_{n_{q}}(t)$ is the \gls{CQI} at \gls{SN} controller at time $t$, and $I_{n_{q}}(t)$ is the estimated interference power. We consider $\nu (t)$ and $w(t)$ as Gaussian noise with known variance $\Omega$ and $R$ respectively. In this work, we consider the evolution The variance ${\Omega}$ represents the combination of the noise variance related to the scheduling of neighboring SN and interference modeling noise. Whereas, $R$ represents the quantization and dequantization noise while mapping effective \gls{SINR} to \gls{CQI}.  Here, the function $\tilde{g} = Q \circ g$ is the function composition of \gls{SINR} mapping using \gls{EESM}/\gls{MIESM} after \gls{SINR} quantization. The dynamics of interference referring to the previous \gls{TTI} is defined by function $f(.)$. The variance of $\tilde{g}$ arises from the product of two Gaussian distributions, yielding a Gaussian distribution with a variance of $ R = \frac{\sigma_{q}^{2} \cdot \sigma_{g}^{2}}{\sigma_{q}^{2} + \sigma_{g}^{2}}$, where $\sigma_{q}$ and $\sigma_{g}$ are variance associated with $Q$ and $g$ \cite{bromiley2003products}.


\section{Extended Kalman Filter-based Predictor}

In this paper, we aim to predict interference at the \gls{SN} controller utilizing only \gls{CQI} data. In every time $t$, \gls{EKF} predicts  $I_{n_q}(t)$ utilizing previous prediction $I_{n_q}(t-1)$ and new observed \gls{CQI} $y_{n_q}(t)$. First of all, we linearized the nonlinear relationship of \cref{eq:1}, which uses the previous prediction such that it exploits correlation due to small-scale fading, which is the main factor for correlation. The correlation of small-scale fading can be approximated by zeroth-order modified Bessel function \(J_{0}(w_{d} \cdot \tau)\), where $w_{d}$ is Doppler spread and $\tau$ is the duration of \gls{TTI} for Rayleigh fading \cite{xiao2006novel}. In the case of Rice fading, the envelope of the \gls{PDF} can be represented by the zeroth-order modified Bessel function \(J_{0}(2 z \sqrt{K(1+K)})\), where $K$  and $z$ are rice factor and fading envelope respectively \cite{xiao2006novel}. This paper exclusively focuses on the Bessel function related to Rayleigh fading, leaving the dynamics between Rice and Rayleigh fading as an open topic for further investigation. By considering a correlation matching criterion, the coefficient for linearization with predicted interference for previous \gls{TTI} $\hat{I}_{n_{q}}(t-1)$ can be related by $\alpha_{b} = J_{0}(w_{d} \cdot \tau)$ \cite{ghandour2012use}. The linearized model is considered as $\hat{I}_{{n_{q}}}(t)= \alpha_{b} \hat{I}_{{n_{q}}}(t-2) + (1- \alpha_{b}) \hat{I}_{{n_{q}}}(t-1)$. Moreover, for linearizing \cref{eq:2}, we consider that the received \gls{CQI} is a wideband and dequantized value from the \gls{CQI}. The estimated \gls{SINR} with quantization error can be linked with interference by \cref{eq:sinr}. We use the Jacobian to linearize this model as 
\begin{align}
    G(t): = \frac{\partial {\gamma}_{n_{q}}(t)}{\partial \hat{I}_{n_{q}}(t)},
\end{align}
which simplifies the impact of changes in interference in \gls{CQI}. The proposed method operates through a simple two-step process: prediction and update. In prediction step, 



\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{images/block_diagram_1.png}
    \caption{Proposed Link Adaptation for In-X \gls{SN}}
    \label{Fig:la_schemetics}
\end{figure}





In this work, we aim to predict interference at the \gls{SN} controller using only \gls{CQI} data. To predict interference, denoted as $I_{n_q}(t)$, from observed \gls{CQI} $y_{n_q}(t)$, we employ an Extended Kalman filter. First of all, we linearize the nonlinear relationship of \cref{eq:1}.  Interfering links, expected to have a lower \gls{LOS} probability due to spatial distance between interferers and the receiver, indirectly favor interference following a Rayleigh distribution. This paper exclusively focuses on the Bessel function related to Rayleigh fading, leaving the dynamics between Rice and Rayleigh fading as an open topic for further investigation. By considering a correlation matching criterion, the coefficient for linearization with predicted interference for previous \gls{TTI} $\hat{I}_{n_{q}}(t-1)$ can be related by $\alpha_{b} = J_{0}(w_{d} \cdot \tau)$ \cite{ghandour2012use}. The linearized model is considered as $\hat{I}_{{n_{q}}}(t)= \alpha_{b} \hat{I}_{{n_{q}}}(t-2) + (1- \alpha_{b}) \hat{I}_{{n_{q}}}(t-1)$. Moreover, for linearizing \cref{eq:2}, we consider that the received \gls{CQI} is a wideband and dequantized value from the \gls{CQI}. The estimated \gls{SINR} with quantization error can be linked with interference by \cref{eq:sinr}. We use the Jacobian to linearize this model as 
\begin{align}
    G(t): = \frac{\partial {\gamma}_{n_{q}}(t)}{\partial \hat{I}_{n_{q}}(t)},
\end{align}
which simplifies the impact of changes in interference in \gls{CQI}. 


Moreover, it is observed that small-scale fading predominantly influences the channel correlation, which can be described using the zeroth-order modified Bessel function \(J_{0}(w_{d} \cdot \tau)\), where $w_{d}$ is Doppler spread and $\tau$ is the duration of \gls{TTI} for Rayleigh fading \cite{xiao2006novel}. In the case of Rice fading, the envelope of the \gls{PDF} can be represented by the zeroth-order modified Bessel function \(J_{0}(2 z \sqrt{K(1+K)})\), where $K$  and $z$ are rice factor and fading envelope respectively \cite{xiao2006novel}.

As we consider dequantized data as input, we need to reflect quantization, compression and reconstruction error in terms of variance $R$. We have considered that the variance $R$ arises from the combination of quantization error, with variance $\mathcal{N}(0,\sigma_{q}^{2})$, and process noise, with variance $\mathcal{N}(0,\sigma_{g}^{2})$. We consider the variance associated with quantization error as $\mathcal{N}(0,\sigma_{q}^{2})$ for uniform quantization of minimum and maximum \gls{SINR}. As the quantization method may vary depending on the use case specification, the variance can be replaced by the respective quantization error variance determined by the selected quantization technique. After linearizing the model, we proceed with the prediction using the Kalman filter \cite{kay1993fundamentals}.

We generate the \gls{CQI} $y_{n_q}(t)$ based on the \gls{SINR}, computed using $Q(g(\gamma_{n_q}(t)))$, where 
\begin{align}\label{eq:sinr}
&\gamma_{n_q}(t) = \dfrac{S_{n_q}(t)}{I_{n_{q}}(t)+w}   
\end{align}
 with $w$ representing thermal noise power. The symbol $S_{n_q}(t)$ is signal power while transmitting a packet from \gls{SN} controller to \gls{SA} pair for downlink and \gls{SA} pair to \gls{SN} controller.

The overall interference prediction can be summarized in the following algorithm:

\begin{algorithm}
\caption{Extended Kalman Filter for Interference Prediction \cite{kay1993fundamentals}}
\label{algo:proposed_algo}
\begin{algorithmic}[1]
\State \textbf{Input:} Received CQI $y_{n_q}(t)$ at SN controller
\For{$i = 1, \dots$}
\State Prediction:  $\hat{I}_{n_{q}}(t| t-1 ) = \alpha_{b}\cdot \hat{I}_{n_{q}}(t-1 | t-1 )+ (1-\alpha_{b})\cdot \hat{I}_{n_{q}}(t-1 | t-2 )$
\State Minimum Prediction MSE: ${\Sigma }(t \big| t-1 ) = {\alpha_{b}}^2 \cdot {\Sigma }(t-1 \big| t-1) +{Q}$
\State Measurement residual: ${S}(t \big| t-1 ) = {{G(t)}}\cdot {\Sigma }(t \big| t-1) \cdot {{G(t)}}^\top +R$
\State Kalman Gain:  $\mathcal{K}(t)=\dfrac{{{\Sigma }}(t \big| t-1 )\cdot { {G}}}{ { {S}}^{-1}(t \big| t-1 )}$
\State Update State estimate: $\Delta  {y}_{n_{q}}(t)= {y}_{n_{q}}(t)-\hat{ {y}}_{n_{q}}(t \big| t-1 )$
\State  Correction: $\hat{I}_{n_{q}} (t | t)= \hat{I}_{n_{q}}(t | t-1)+{\mathcal{K}}(t)\cdot {\Delta} {y}_{n_{q}}(t)$
\State Minimum MSE: $\Sigma(t | t) = (1-\mathcal{K}(t)\cdot  G(t))\cdot {\Sigma }(t \big| t-1)$
\EndFor
\end{algorithmic}
\end{algorithm}
The proposed method operates through a simple two-step process: prediction and correction. Initially, it uses current information to predict the future state of the system $\hat{I}_{n_{q}}(t| t-1 )$ and its uncertainty $\boldsymbol{\Sigma }(t | t-1 )$. Then, when new data comes in, it measures the difference $\hat{y}_{n_{q}}(t | t-1 )$ between what was predicted and what actually happened. This process helps adjust the predictions to be more accurate, combining what was expected with the latest measurements. Leveraging the calculated Kalman Gain $\mathcal{K}(t)$, the \gls{EKF} adjusts this residual to refine the state estimate $\hat{I}_{n_{q}} (t | t)$ and its uncertainty $\Sigma(t | t)$, effectively integrating the predictive model with incoming data. This iterative mechanism, which adeptly minimizes estimation errors through a dynamic equilibrium between model forecasts and measurement accuracy, establishes the \gls{EKF} as an essential tool for achieving optimal state estimation in real-time and dynamic systems. Through the continuous application of these steps, the \gls{EKF} persistently refines its state estimates, thereby ensuring high precision in the system's state approximation over time. This ongoing process of predicting interference and subsequently refining based on newly observed \gls{CQI} enables the \gls{EKF} to accurately capture the dynamic nature of interference over time.

==> extras/src_old/conclusion_old.tex <==
\section{Conclusion}

In this research, we propose an online and unsupervised interference prediction technique, the \gls{EKF} predictor, capable of inferring and predicting dynamic interference based on available \gls{CSI}—specifically, the CQI at the \gls{SN} controller. Despite being online and utilizing only two samples of previously predicted interference, the performance in terms of prediction error is comparable with \gls{LSTM} and optimal \gls{LA}, despite discrepancies in selecting variances associated with quantization, compression, and reconstruction. This suggests that the proposed low-complexity state-space modeling has the potential to achieve comparable performance to machine learning methods. Furthermore, further investigation into unknown variances remains an open topic.

==> extras/src_old/introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}

There is an increasing demand to integrate emerging industrial vertical services as part of the future \gls{6G} communication infrastructure. The ``Network-of-Networks" concept has been identified as a potential solution, where a vertical can be integrated as a \gls{SN}~\cite{hoffmann2023secure}. A typical \gls{SN} comprises of an \gls{AP} and several \glspl{UE} either connected to the controller or communicating among themselves. The \gls{SN} devices are envisioned to operate in short-ranges with \gls{HRLLC} traffic requirements. More information on common \gls{SN} use-cases and deployment scenarios can be found in~\cite{berardinelli2021extreme}. 

\gls{IM} has been identified as one of the major technical challenges involved in real-time \gls{SN} deployments. From an air-interface perspective, \gls{IM} can be achieved through a combination of resource allocation and \gls{LA}. While the former focuses more on appropriate radio resource management, \gls{IM} through \gls{LA} involves exploiting the underlying transmission link characteristics. In this work, we focus on improving the \gls{LA} aspects of \gls{IM} for industrial \gls{SN} devices.

The baseline \gls{LA} scheme used for \gls{URLLC} traffic involves \gls{MCS} selection based on the \gls{CQI} report and ACK/NACK feedback. Here, \gls{CQI} report is a quantized information characterizing the transmission link. Such schemes are not readily applicable for \gls{IM} in \glspl{SN} for the following reasons. Firstly, short packets of \gls{HRLLC} trafﬁc occupy only a fraction of the physical resources in a \gls{TTI}. This results in a rapidly varying interference among \glspl{SN}, which can be particularly challenging to track in real-time. Added to this, the delay involved in \gls{CQI} reporting mechanisms~\cite{ramezani2021cqi} only makes it worse. Secondly, extreme low latency requirements of \glspl{SN} impose stringent limitations on packet retransmissions~\textemdash~oftentimes limiting it to only one retransmission. Such requirements cannot be met with the baseline described above due to extremely dense \gls{SN} deployments.

In this work, we model and propose an interference prediction mechanism at a \textit{\gls{SN} controller} to assist the \gls{LA} in achieving desired reliability requirements. This is in contrast to the existing literature where interference prediction/estimation is  performed at \gls{SA}-pairs. For instance, the authors in~\cite{pocovi2018joint} employ a low-pass first-order IIR filter \glspl{IPV}, which are then  . Xiang et al. utilized a Wiener filter with extrapolation in \cite{xu2013improving}. The authors of \cite{brighente2020interference} introduced a low-complexity version for interference prediction using kernel-based probability density. Moreover, in \cite{mahmood2020predictive}, a discrete state-space discrete-time Markov chain has been utilized for interference prediction. In that work, the area under the distribution is defined as $\eta$, which is used to utilize the tail statistics of the interference distribution. In our recent work, we proposed prediction methods using historical interference power values, Wiener, \gls{LSTM}, and Federated LSTM-based predictor \cite{pramesh2024int,gautam2023co} for In-X \glspl{SN}, assuming that the interference power value is perfectly known. For our proposed methods, we use estimated interference power values, which do not require information about the distribution of interference including the minimum and maximum \gls{INR} like \cite{mahmood2020predictive}. In this work, we consider moving average and LSTM-based predictor as baseline methods.

% Our proposed method considers the prediction of interference is performed at the \gls{SN} controller and the available data is  CQI only. The CQI is generated uniformly quantized from estimate  \gls{SINR} into $5$ bit with 32 \gls{MCS} as specified in \cite{3gpp2018physical}. We assume that \glspl{CQI} is only the available data with \gls{SN} controller, which carries the information about the dynamics of channel statics together with mobility and short packet traffic.  We propose the technique to predict interference at the next transmit time interval \gls{TTI} from the currently observed CQI. Learning these dynamics helps to mitigate the effect of CQI expiry and is anticipated to help achieve effective MCS selection \cite{ramezani2021cqi}. Hence, we propose an extended Kalman filter for interference prediction by observing CQI at the \gls{SN} controller which works as unsupervised learning fashion. 
The contributions of this research are summarized here:

\textit{\textbf{Contribution 1:}}  The proposed state-space modeling employing the \gls{EKF} predicts interference in an online, unsupervised manner by leveraging accessible CSI data at the \gls{SN} controller, specifically the \gls{CQI}. Furthermore, this state-space prediction framework accounts for quantization, compression, reconstruction errors, and process noise. It also integrates the correlation coefficient of small-scale fading to bolster predictor performance. This method doesn't need the interference power value, i.e., a label at the \gls{SN} controller, which makes the cost associated with transferring that interference data redundant.

\textit{\textbf{Contribution 2:}} The predicted interference has been utilized for link adaptation purposes to select the optimal \gls{MCS}, ensuring the target \gls{BLER}, which has been considered as a reliability measure. The efficacy of the proposed method is evaluated using a spatially consistent \gls{3GPP} channel model for indoor factory scenarios. Moreover, this approach does not require \gls{ACK}/\gls{NACK} feedback for selecting \gls{MCS} from estimated \gls{SINR}, unlike \gls{OLLA}, thus being well suited for extremely low latency traffic.



==> extras/src_old/problemformulation_old.tex <==
\section{Problem Description}
\label{sec.probformulation}

The \gls{LA} problem involves appropriate selection of \gls{MCS} values subject to reliability constraints. As mentioned in section~\ref{sec:systemmodel}, a \gls{SN} controller performs \gls{MCS} selection based on the \gls{CQI} report received from the \gls{SA} pairs associated with it. Formally, the \gls{LA} problem for the $m^{\text{th}}$ \gls{SA}-pair of the $n^{\text{th}}$ \gls{SN} at \gls{TTI} $t$ can be expressed as:
\begin{multline}
\label{eq:laprob}
\phi_{(n,m)}^*(t) = \sup\{R(\phi_{(n,m)}(t)) | \varepsilon(\phi_{(n,m)}(t)) \leq \Bar{\varepsilon}\},
\end{multline}
where, $\phi_{(n,m)}^*(t) \in \Phi$ is the optimal \gls{MCS} value with $\Phi$ being the set of all feasible \gls{MCS} values. The quantity $R(.)$ denotes the achievable ergodic rate of the $m^{\text{th}}$ \gls{SA} pair. Finally $\varepsilon(t)$ and $\Bar{\varepsilon}$ represent the achieved \gls{BLER} and target \gls{BLER} values, respectively.

Following practical challenges arise while solving~\eqref{eq:laprob}:
\begin{enumerate}[label=(\alph*)]
    \item The interference experienced by \gls{SA}-pairs is not sufficiently reflected in~\eqref{eq:laprob} due to the function characterizing the \gls{ESM} mechanisms and limited quantization levels characterizing the \gls{CQI} report.
    \item Secondly, a controller is more likely to perform \gls{MCS} selection based on outdated \gls{CQI} and subsequently interference information due to inherent protocol overhead and transmission delays involved.
\end{enumerate}

While (a) and (b) are not just specific to \gls{LA} for \glspl{SN}, not accounting for them in~\eqref{eq:laprob} can have a detrimental effect on the overall latency and reliability requirements, especially in \glspl{SN}. A straightforward way to include interference information in~\eqref{eq:laprob} is by explicitly measuring the \glspl{IPV} at an \gls{SA}-pair and sending them back to the associated controller. However, this is impractical in ultra dense \glspl{SN} since it introduces additional signalling and computational overhead. In this work, we resort to an online signalling-free interference prediction scheme by exploiting the \gls{CQI} available at the controller, which we describe in the next section. 


==> extras/src_old/proposedpredictor_old.tex <==
\section{Proposed Approach}
\label{sec:proposedapproach}

Prior to delving into details of the proposed interference prediction scheme, in this section, we first present a generalized \gls{DSSM} for \glspl{IPV} modeled w.r.t the \gls{CQI} report.

\subsection{\gls{DSSM} Characterization}
An important aspect of the \gls{CQI} report is that it implicitly captures the interference information, even when it is subjected to several estimation/inference and modeling perturbations both at the \gls{SA}-pairs and the controller. Secondly, \glspl{IPV} demonstrate correlation across \glspl{TTI} due to the underlying channel model. Taking advantage of these aspects, the inter-dependencies between \glspl{IPV} and the available \gls{CQI} reports can be characterized using a general-\gls{DSSM} at the controller. Formally, the \gls{DSSM} at the $n^{\text{th}}$ controller can be expressed as follows:
\begin{subequations}
\label{eq:dssm}
\begin{align}
    &\pmb{I}_n(t) := f(\pmb{I}_n(t-1), \pmb{\nu}(t)), \label{eq:dssma} \\
    &\pmb{Y}_n(t) := g(\pmb{I}_n(t), \pmb{u}(t)). \label{eq:dssmb}
\end{align}
\end{subequations}
Here,~\eqref{eq:dssma} represents a process model describing the dynamic evolution of \gls{IPV} over the \glspl{TTI}, where $\pmb{I}_n(t)$ is a vector of \glspl{IPV}, modeled as hidden/latent states of the \gls{DSSM}. Similarly,~\eqref{eq:dssmb} corresponds to a measurement model relating the vector containing \gls{CQI} reports of the \gls{SA}-pairs to \glspl{IPV}. The \gls{CQI} reports or observations of the measurement model are succinctly represented by the vector $\pmb{Y}_n(t)$. Furthermore, $f(.)$ and $g(.)$ denote non-linear functions characterizing the hidden state transition and observations corresponding to the process and measurement models, respectively. Finally, $\pmb{\nu}(t)$ and $\pmb{u}(t)$ correspond to process and measurement noise, respectively. Here, we would like to highlight that unlike existing works from section~\ref{sec:introduction}, the \gls{DSSM} in~\eqref{eq:dssm} considers the full range of the p.d.f of \glspl{IPV} and not just the tail probabilities. 

\subsection{\gls{EKF}-based Interference Prediction}

An important point to notice in~\eqref{eq:dssmb} is that we consider the \gls{CQI} of $Y_{(n,m)}(t)$ of the $m^{\text{th}}$ \gls{SA}-pair  We consider $\nu(t)$ and $u(t)$ as Gaussian noise with known variance $\sigma_{f}$ and $\sigma_{g}$ respectively. The variance $\sigma_{f}$ represents the combination of the noise variance related to the scheduling of neighboring SN and interference modeling noise. Whereas, $\sigma_{g}$ represents the quantization and dequantization noise while mapping \gls{eSNR} to \gls{CQI}. Here, the function $g = g_{1} \circ g_{2}$ is the function composition of \gls{eSNR} mapping using \gls{ESM} after \gls{SINR} quantization.
% The dynamics of interference referring to the previous \gls{TTI} is defined by function $f(.)$. 
The variance of $g$ arises from the product of two Gaussian distributions, yielding a Gaussian distribution with a variance \cite{bromiley2003products} as 
\begin{align}
 \sigma_{g} = \frac{\sigma_{g_{1}}^{2} \cdot \sigma_{g_{2}}^{2}}{\sigma_{g_{1}}^{2} + \sigma_{g_{2}}^{2}},
\end{align}
where $\sigma_{g_{1}}$ and $\sigma_{g_{2}}$ are variance associated with $g_1$ and $g_2$. In this work, we consider the state evolution of \glspl{IPV} and the measurement model transformation to be linear and expressed as follows:
\begin{align}
    f(\mathbf{I}_{n}(t-1)) \approx  \mathbf{F} \cdot \mathbf{I}_{n}(t-1) , \  g(I_{n}(t)) \approx G(t) \cdot I_{n}(t).
\end{align}

We consider the state evolution in \cref{eq:dssma} to be due to small-scale fading as the primary source of correlation, and thus, we have incorporated its approximate solution accordingly. The correlation due to small-scale fading can be approximated by zeroth-order modified Bessel function $B_{0}(w_{d} \cdot \tau)$, where $w_{d}$ is Doppler spread and $\tau$ is the duration of \gls{TTI} for Rayleigh fading \cite{xiao2006novel}. In the case of Rice fading, the envelope of the \gls{PDF} can be represented by the zeroth-order modified Bessel function $B_{0}(2 z \sqrt{K(1+K)})$, where $K$  and $z$ are rice factor and fading envelope respectively \cite{xiao2006novel}. In this work, we focus on the Bessel function related to Rayleigh fading, leaving the dynamics between Rice and Rayleigh fading as an open topic for further investigation. By adopting a correlation matching criterion \cite{ghandour2012use}, the state evolution vector for predicted interference at time $t$ utilizing previously predicted interferences at $t-1$ and $t-2$ \glspl{TTI}, is represented as  $\mathbf{F} =  [\alpha_{b},1- \alpha_{b}]$, where $\alpha_{b} = B_{0}(w_{d} \cdot \tau)$. The transformation can be expressed as  
\begin{align}
    \hat{I}_{{n}}(t) \approx \alpha_{b} \hat{I}_{{n}}(t-2) + (1- \alpha_{b}) \hat{I}_{{n}}(t-1) : =  \textbf{F} \cdot \mathbf{\hat{I}}_{n}(t-1).
\end{align}
where $\mathbf{\hat{I}}_{n}(t-1) = [\hat{I}_{{n}}(t-1),\hat{I}_{{n}}(t-2)]^\top$ is previously predicted \glspl{IPV}. The latent variable interference is related to the received \gls{CQI}, which is a quantized value resulting from \gls{SINR} mapping via \cref{eq:sinr}. Considering wideband \gls{CQI}, and the function $g(\cdot)$ being differentiable in a time-dependent manner, we express this using partial derivatives through the Jacobian as:
\begin{align}
    G(t): = J_{I_{n}}(g(t)),
\end{align}
thus simplifying the evaluation of interference-induced changes in \gls{CQI}.



==> extras/src_old/simulations_old.tex <==
\section{Simulation Setup and Analysis}
\subsection{Baseline prediction techniques}
We have considered three methods: the moving average predictor, \gls{LSTM}-based predictor, and Genie predictor, which aid in achieving optimal \gls{LA}. Among all three methods, we assume perfect knowledge of the interference power values is known to predictor instead of \gls{CQI} for both the moving average predictor and the \gls{LSTM}-based predictor.
\subsubsection{Moving Average Predictor}
 The baseline method is the weighted average-based interference estimator, which is used in \gls{LA} for traditional \gls{eMBB} services. The interference measured/estimated at time $t-1$ is filtered with a low-pass first-order \gls{IIR} filter to predict the interference at $t$  \cite{mahmood2020predictive}:
 \begin{equation} \label{eq:7}
 \hat{I}_{{n}}(t)= \alpha I_{{n}}(t-2) + (1- \alpha) \hat{I}_{{n}}(t-1)
\end{equation}
where $0<\alpha < 1$ is the forgetting factor of the filter. This method illustrates the effectiveness of mean prediction.
\subsubsection{LSTM-based Predictor}
The \gls{LSTM}-based interference predictor was proposed in our recent work \cite{gautam2023co} for the In-X subnetwork.  The interference power vector $\mathbf{I}_{{n}}$ is considered as the input for the \gls{LSTM} model. The data is restructured with a sliding window $\Omega_{W}$ and a step size of $\Omega_{p}$. The task is to predict the interference of the $n$th \gls{SN} at time $t+1$ by utilizing the IP vector $\mathbf{I}_{n}(t) = [I_{n}(t-1), \dotsc, I_{n}(t -\Omega_{w}-1)]^{T}$ for a trained model of the respective \gls{SA} pair's \glspl{IPV} as 
\begin{align} \label{eq:onetoone}
\hat{I}_{n}(t)= f_{\textbf{w}}(\mathbf{I}_{n}(t-1)^{T}),
\end{align}
where $\textbf{w}$ is trained \gls{LSTM} model parameter. The detailed discussion and related results can be found in \cite{gautam2023co}. Unlike this work, \cite{gautam2023co} assumes that the interference power value is known at the \gls{SN} controller, and considered noise free.
\subsubsection{Optimal \gls{LA}}
Assuming that the \gls{SINR} is perfectly known a priori in the \gls{SN} controller, it can select the proper \gls{MCS} based on the defined target \gls{BLER} $\varepsilon_{\text{target}}$ \cite{alonzo2020urllc}.

\subsection{Simulation Setup}

The simulation assumptions regarding \gls{SN} deployment, channel parameters, and \gls{EKF} parameters are detailed in \cref{table:2}. We assume that $16$ uniformly distributed \glspl{SN} are deployed in a confined area of $20 \times 20 \, \text{m}^2$, each moving at constant velocity $2 \, \text{m/s}$ in a random direction with $\theta$ drawn from a uniform distribution between $0$ and $2 \pi$. We consider that the one \gls{SA} pair is distributed according to a binomial point process whose p.d.f is given by $(\pi r^{2})^{-1}$ in a disc of radius $r =2$.  The \glspl{SN} follow the \gls{RDMM}. Moreover, as these \glspl{SN} are mobile, there is a possibility that receivers or potential interferers may be in either \gls{LOS} or \gls{NLOS} conditions. We consider a spatially consistent \gls{3GPP} channel model related to the \gls{InF-DL}, which is suitable for our considered use case. The proposed interference model accounts for the \gls{LOS} probability as those \glspl{SN} move in dynamically, which has the ability to adopt the possibility of change in \gls{LOS} and \gls{NLOS}. The respective parameter related to free space path loss and shadowing for \gls{LOS} and \gls{NLOS} has been used from \cite{3gpp2018study}. The parameters associated with the channel are specified in \cref{table:2}. For the \gls{LSTM} method, the train and test data are restructured with a sliding window of size $\Omega_{W}=30$ and a step size of $\Omega_{p}=1$. This ensures that for prediction, this technique utilizes $\Omega_{W}$ historical interference power values and predicts for the next time instance. The \gls{LSTM} model is trained as specified in \cite{gautam2023co} for 200 epochs. The performance is compared in terms of the achieved \gls{BLER} based on predicted interference from these techniques. However, \gls{EKF} utilizes coefficients obtained from a modified Bessel function to weigh previously predicted interference and refines the prediction when new \gls{CQI} is observed. We assume uniform quantization with an identical step size of $\Delta$ for $|\Phi| = 29$ \gls{MCS} in between the minimum and maximum of \gls{SINR} in this work.  To ensure a fair comparison between the proposed method and \gls{LSTM}, we utilized $20,000$ predicted interference power values, selected from the unseen test data comprising $20\%$ of the total $100,000$ samples, for evaluation against the \gls{LSTM}-based predictor.
\begin{table}
\centering
\caption{ Simulation Setting for interference analysis and estimation}
\label{table:2}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{ll} \hline
\textbf{Parameter}                                          & \textbf{Value}~  \\ \hline
Deployment Parameter                                       \\ \hline
Number of subnetworks , $|\mathcal{N}|$                                   & 16               \\ 
Number of sensor-actuator pair, $|\mathcal{M}|$                           & 1                \\
Interfering subnetworks, $|\mathcal{K}|$                           & 4                \\

Deployment Area & $20 \times 20$            \\ \hline
Mobility Parameter                                        \\ \hline
Mobility Model                                              & RDMM             \\
Cell Radius, r                                    & 2 [m]            \\
Velocity, $v$                                             & 2 [m/s]          \\
Minimum distance, $d$                                     & 4 [m]            \\ \hline
Channel Parameter   \cite{3gpp2018study}                                        \\ \hline
Pathloss               & \gls{3GPP} \gls{InF-DL}            \\
Shadow fading standard deviation                            & 4 (for LOS)$|$7.2(for NLOS) [dB]        \\
Decorrelation distance, $\delta$           & 10 [m]            \\ \hline
Carrier frequency, $f_{c}$                             & 6 [GHz]         \\
Number of available  Channel, $N_{ch}$                           & 4                \\
Frequency reuse                            & $1/4$                \\
\hline
EKF Parameters                                          \\ \hline
Quantization variance, $ \sigma_{g_1}^{2}$          &  $\dfrac{\Delta^{2}}{12\times |\Phi|}$    \cite{easton2010fundamentals}      \\ 
Process noise variance, $\sigma_{g_2}^{2}$       & $2\cdot{10}^{-9}$           \\ 
Noise Factor, $NF$       & $10$ dB           \\ 
Noise Bandwidth, $BW$         & $50$ Mhz           \\
Variance, $\sigma_{f}$          & $0.0042$           \\
\hline
\end{tabular}}
\end{table}
\subsection{Numerical Results}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\linewidth]{images/plot.eps}
%     \caption{Prediction of interference for a fixed time step~(test data)}
%     \label{fig:predictiontrajectory}
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{images/RESULTS/absoulute_error_1_sub.eps}
    \caption{ECDF of Relative Absolute Error}
    \label{fig:predictiontrajectory}
\end{figure}
We evaluated the prediction error in terms of \gls{ECDF} of relative absolute error. The relative absolute prediction error can be defined as  \cite{pramesh2024int}:
 \begin{equation}\label{eq:rerr}
     R_{err}[k]=|(I_{n}(t)-\hat{I}_{n}(t))/I_{n}(t)|.
 \end{equation}
\cref{fig:predictiontrajectory} illustrates the distribution of relative absolute prediction error. It demonstrates that the \gls{EKF} outperforms the moving average predictor with approximately $10$ dB lower prediction error. Moreover, as an online and unsupervised learning method, it leads to a prediction error of $1.31$ dB at $50$th percentile as compared to \gls{LSTM}-based predictor. This highlights how state-space modeling of interference at the \gls{SN} controller without labels helps achieve comparable performances with \gls{LSTM}, which is trained offline with a sliding window size of $\Omega_{W} = 30$. 
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{images/RESULTS/ecdf_1_sub.eps}
    \caption{\gls{ECDF} of Achieved \gls{BLER}}
    \label{fig:bler_ecdf}
\end{figure}
It is necessary to analyze the discrepancy in the performance of those predictors for \gls{IM} in terms of achievable \gls{BLER} by selecting \gls{MCS} based on predicted interference. In this work, we generate the lookup table with \gls{BLER} vs range of \glspl{SNR} for specific \gls{MCS} with specific \gls{MO} and \gls{CR} based on Table 5.1.3.1-3 from \cite{3gpp2018physical} by considering packet size of $20$ bytes \cite{alonzo2020urllc}. We use \gls{EKF} to predict the interference from \gls{CQI}. We utilize the predicted interference to adjust the \gls{SINR} for the next \gls{TTI} considering the $S_{(n,m)}$ is perfectly known due to short-range communication, along with the fixed position of the \gls{SN} controller and \gls{SA} pair. The adjusted \gls{SINR} is used to select the optimal \gls{MCS} $\phi_{(n,m)}^*(t)$ from a lookup table, as detailed in \cref{sec.probformulation}. The achievable \gls{BLER} is then computed using the selected \gls{MCS} and the true \gls{SINR}, referencing the \gls{MCS} table. This analysis provides insights into the discrepancies arising from the improper selection of \gls{MCS} due to prediction errors in both the proposed and baseline methods.

% Once the \gls{MCS} is selected from the predicted interference, \gls{BLER} is retrieved from the \gls{MCS} look-up table corresponding to the predicted \gls{SINR}, allowing us to assess the difference between the targeted and observed \gls{BLER}, reflecting the comparison between the actual and predicted \gls{SINR}. 

The results in \cref{fig:bler_ecdf} illustrate that based on the selected \gls{MCS}, the \gls{EKF} achieves the target \gls{BLER} $10^{-5}$ for $95\%$ of the time. The \gls{EKF} and \gls{LSTM} both effectively predict interference, achieving \glspl{BLER} comparable to those of optimal \gls{LA}. In contrast, the moving average predictor exhibits significant deviations. Notably, optimal \gls{LA} tends to slightly outperform the target \gls{BLER} due to the limited number of \glspl{MCS} available as shown in  Fig.~1 of \cite{alonzo2020urllc}. In addition, we evaluated three predictors while varying the target BLER with respect to optimal LA, as depicted in \cref{fig:blercomparison}. The optimal LA, while practically infeasible, provides insight into the upper bound achievable by appropriately selecting the \gls{MCS}. Our findings indicate that the EKF can achieve the target BLER with a slight margin for the $95\%$ percentile among $20,000$ test samples, as the target BLER increases. Thus, while the LSTM-based predictor may offer slightly better performance, the EKF predictor remains a valuable approach, providing a balance between prediction quality and computational efficiency.
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{images/RESULTS/bler_1_sub.eps}
    \caption{Achieved BLER for varying target BLER}
    \label{fig:blercomparison}
\end{figure}

==> extras/src_old/systemmodel_old.tex <==
\section{System Model}
\label{sec:systemmodel}

Let $\mathscr{N} = \{1,2,\ldots,N\},~|\mathscr{N}|=N$, denote the set of \glspl{SN} distributed according to a uniform random variable in a confined area $\mathscr{A}$. Each \gls{SN} $n \in \mathcal{N}$ consists of a single controller serving $\mathscr{M} = \{1,2,\ldots,M\}, |\mathscr{M}|=M$ \gls{SA}-pairs in the \gls{DL}. Since a controller uniquely identifies a \gls{SN}, the terms \gls{SN} and controller are used interchangeably in this document. Each \gls{SN} is assumed to be moving with constant velocity $v$ with the direction defined by $\theta \in [0,2\pi]$ (see \cref{fig:subnet_layout}). Moreover, \glspl{SN} are configured to maintain a minimum separation distance of $d_{sep}$.
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{images/final_layout.png}
    \caption{Illustrative example of the \gls{SN} deployment.}
    \label{fig:subnet_layout}
\end{figure}

We assume a slotted time operation where each slot or a \gls{TTI} is denoted by $t \in \mathbb{N}$. The total available bandwidth $B$ is partitioned into $N_{ch},~N_{ch} <\!< N$ sub-bands and a \gls{SN} is assumed to operate in the TDD mode. Furthermore, only a single sub-band at any given \gls{TTI} $t$; however, multiple \glspl{SN} can be allocated to the same sub-band. This results in an inter-\gls{SN} interference scenario. Moreover, due the short-range operations of the \glspl{SN}, we assume that all \gls{SA}-pairs in a \gls{SN} experience \textit{same} interference. This is a valid assumption for In-body/In-Vehicle \gls{SN} scenarios. On the other hand, we assume that there is no intra-\gls{SN} interference. This can be achieved by using a scheduler at the controller, which schedules the \gls{SA}-pairs in a near-orthogonal fashion~\cite{skapoor2018distributedscheduling}. Furthermore, we model the \gls{SN} traffic according to an i.i.d Bernoulli random variable w.l.o.g, i.e., a controller either has a packet to transmit or remains idle during a \gls{TTI} $t$.

Following operations ensue in a \gls{SN} to successfully perform \gls{LA} for \gls{DL} transmissions. The controller transmits reference signals, which are used to estimate the \gls{SINR} by the associated \gls{SA}-pairs either for all the $N_{ch}$ or $\Tilde{N}_{ch} <\! N_{ch}$ sub-bands. The estimated \gls{SINR} is converted to \gls{eSNR} using an \gls{ESM} mechanism~\cite{pocovi2017mac}. The \gls{eSNR} value is used to prepare the \gls{CQI} report using predefined look-up tables, which is then sent to the controller in a periodic/aperiodic manner. At the controller, the received \gls{CQI} is mapped to the corresponding \gls{SINR} estimate using a look-up table before performing \gls{LA}. The \gls{SINR} estimate of an \gls{SA}-pair, denoted by $\hat{\gamma}_{(n,m)}$, can be written as:
\begin{align}
\label{eq:sinr}
&\hat{\gamma}_{(n,m)}(t) := \frac{S_{(n,m)}(t)}{I_{n}(t)+w(t)},
\end{align}
where, $S_{(n,m)}(t)$ denotes the signal power, which is a function of the wireless channel between the $m^{\text{th}}$ \gls{SA}-pair and the $n^{\text{th}}$ controller. The quantity $w(t) \sim \mathcal{N}(0, \sigma_w^2)$ is the thermal noise of the receiver with variance $\sigma_w^2$ assumed to be same for all \gls{SA}-pairs. Finally $I_n(t)$ is the inter-\gls{SN} \gls{IPV} perceived by the $m^{\text{th}}$ \gls{SA}-pair. Notice the difference in subscripts of $S_{(n,m)}(t)$ in the numerator and $I_n(t)$ in the denominator, which is possible due to the assumptions on the interference made above.

In this work, we model $I_n(t)$ based on the spatially consistent \gls{3GPP} channel model~\cite{3gpp2020study}, and formally express it as:
\begin{multline}
\label{eq:interferencemodeling}
I_{n}(t) := \sum_{n^{\prime} \in \hat{\mathscr{N}}(t)\setminus\{n\}} \chi_{n^{\prime}}(t) \cdot \biggl(\beta |H_{LOS,n^{\prime}}(t)|^2+ \\ \sqrt{(1- \beta^2)} |H_{NLOS,n^{\prime}}(t)|^2\biggr),
\end{multline}
where, $\mathscr{\hat{N}}(t)\subset\mathscr{N}$ denotes the set of all \glspl{SN} operating in the same sub-band at \gls{TTI} $t$. The quantity $\chi_k(t) \sim Ber(p)$ denotes the ON-OFF traffic parameterized by probability $p$. Furthermore, $H_{LOS,n^{\prime}}(t) := h_{LOS,n^{\prime}}(t)\cdot l_{LOS,n^{\prime}}(t)\cdot\zeta_{LOS,n^{\prime}}(t)$ is the consolidated \gls{LOS} channel where $h_{LOS,n^{\prime}}$ is the small-scale fading co-efficient correlated across \glspl{TTI} and following Rician p.d.f; $l_{LOS,n^{\prime}}$ is the path loss component and $\zeta_{LOS,n^{\prime}}$ represents the spatially correlated shadowing effect, which follows a log-normal p.d.f \cite{lu2015effects}. The value $H_{NLOS,n^{\prime}}$ is the consolidated \gls{NLOS} channel defined in a way similar to the \gls{LOS} channel. However, $h_{NLOS,n^{\prime}}$ follows a Rayleigh p.d.f, with the p.d.f of $l_{NLOS,n^{\prime}}$ and $\zeta_{NLOS,n^{\prime}}$ remaining the same as \gls{LOS} channel. The parameter $\beta \in (0,1)$ is a smoothing factor which prevents abrupt fluctuations in the channel response caused due to transitions between \gls{LOS} and \gls{NLOS} conditions \cite{3gpp2020study}. With the system model in place, we next present the problem description in the following section.



==> extras/systemmodel_rev.tex <==
\section{System Model}
\label{sec:systemmodel}

Let $\mathscr{N} = \{1,2,\ldots,N\},~|\mathscr{N}|=N$, denote the set of In-X \glspl{SN} distributed according to a uniform random variable in a confined area $\mathscr{A}$. Each \gls{SN} $n \in \mathscr{N}$ consists of a single \gls{AP} serving $\mathscr{M} = \{1,2,\ldots,M\}, |\mathscr{M}|=M$ \glspl{UE} in the \gls{DL}. Since a \gls{AP} uniquely identifies a \gls{SN}, the terms \gls{SN} and \gls{AP} are used interchangeably in this paper. Each \gls{SN} is assumed to be moving with constant velocity $v$ with the direction defined by $\theta \in [0,2\pi]$ (see \cref{fig:subnet_layout}). Moreover, \glspl{SN} are configured to maintain a minimum separation distance of $d_{\text{sep}}$.
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{images/industrialsn.png}
    \caption{Illustrative example of the \gls{SN} deployment. The respective SA pair has been considered as UE, and \gls{SN} controller as \gls{AP}.}
    \label{fig:subnet_layout}
\end{figure}

We assume a slotted time operation where each slot or a \gls{TTI} is denoted by $t \in \mathbb{N}$. The total available bandwidth $B$ is partitioned into $K,~K <\!< N$ sub-bands and a \gls{SN} is assumed to operate in the TDD mode. Furthermore, an \gls{SN} is assigned to only a single sub-band at any given \gls{TTI} $t$; however, multiple \glspl{SN} can be allocated to the same sub-band. This results in an inter-\gls{SN} interference scenario. Moreover, due the short-range operations of the \glspl{SN}, we assume that all \glspl{UE} in a \gls{SN} experience \textit{same} interference. This is a reasonable assumption for In-body/In-robot \gls{SN} scenarios. On the other hand, we assume that there is no intra-\gls{SN} interference. This can be achieved by using a scheduler at the \gls{AP}, which schedules the \glspl{UE} in a near-orthogonal fashion~\cite{skapoor2018distributedscheduling}. Furthermore, we model the \gls{SN} traffic according to an i.i.d Bernoulli random variable w.l.o.g, i.e., a \gls{AP} either has a packet to transmit or remains idle during a \gls{TTI} $t$.

The following operations ensue in a \gls{SN} to successfully perform \gls{LA} for \gls{DL} transmissions. The \gls{AP} transmits reference signals, which are used to estimate the \gls{SINR} by the associated \glspl{UE} either for all $K$ or $\Tilde{K} <\! K$ sub-bands. The estimated \gls{SINR} is converted to \gls{eSNR} using an \gls{ESM} mechanism~\cite{pocovi2017mac}. The \gls{eSNR} value is used to prepare the \gls{CQI} report using predefined look-up tables, which is then sent to the \gls{AP} in a periodic/aperiodic manner. At the \gls{AP}, the received \gls{CQI} is mapped to the corresponding \gls{SINR} estimate using a look-up table before performing \gls{LA}. The \gls{SINR} estimate of an \gls{UE}, denoted by $\hat{\gamma}_{(n,m)}$, can be written as:
\begin{align}
\label{eq:sinr}
&\hat{\gamma}_{(n,m)}(t) := \frac{S_{(n,m)}(t)}{I_{n}(t)+\sigma_w^2},
\end{align}
where, $S_{(n,m)}(t)$ denotes the signal power, which is a function of the wireless channel between the $m^{\text{th}}$ \gls{UE} and the $n^{\text{th}}$ \gls{AP}. The quantity $\sigma_w^2$ is the receiver noise power, which is assumed to be same for all \glspl{UE} w.l.o.g. Finally $I_n(t)$ is the inter-\gls{SN} \gls{IPV} perceived by the $m^{\text{th}}$ \gls{UE}. Notice the difference in subscripts of $S_{(n,m)}(t)$ in the numerator and $I_n(t)$ in the denominator. This is possible due to the assumptions on the interference presented above.

In this work, we model $I_n(t)$ based on the spatially consistent \gls{3GPP} channel model ~\cite{3gpp2020study}, and formally express it as:
\begin{multline}
\label{eq:interferencemodeling}
I_{n}(t) := \sum_{n^{\prime} \in \hat{\mathscr{N}}(t)\setminus\{n\}}  \chi_{n^{\prime}}(t) \cdot P_{n^{\prime}}(t) \cdot \biggl(\beta |H_{\text{LOS},n^{\prime}}(t)|^2+ \\ \sqrt{(1- \beta^2)} |H_{\text{NLOS},n^{\prime}}(t)|^2\biggr),
\end{multline}
where, $\mathscr{\hat{N}}(t)\subset\mathscr{N}$ denotes the set of all \glspl{SN} operating in the same sub-band at \gls{TTI} $t$. The quantity $\chi_{n^{\prime}}(t) \sim Ber(\rho)$ denotes the ON-OFF traffic parameterized by probability $\rho$. The term $P_{n^{\prime}}(t)$ denotes the transmit power of the interfering \glspl{SN}. Furthermore, $H_{\text{LOS},n^{\prime}}(t) := h_{\text{LOS},n^{\prime}}(t)\cdot l_{\text{LOS},n^{\prime}}(t)\cdot\zeta_{\text{LOS},n^{\prime}}(t)$ is the consolidated \gls{LOS} channel where $h_{LOS,n^{\prime}}$ is the small-scale fading co-efficient correlated across \glspl{TTI} and following Rician \gls{pdf} \cite{xiao2006novel}; $l_{\text{LOS},n^{\prime}}$ is the path loss component \cite{3gpp2020study} and $\zeta_{\text{LOS},n^{\prime}}$ represents the spatially correlated shadowing effect, which follows a log-normal \gls{pdf} \cite{lu2015effects}. The value $H_{\text{NLOS},n^{\prime}}$ is the consolidated \gls{NLOS} channel defined in a way similar to the \gls{LOS} channel. The correlated small scale fading across \gls{TTI} with rayleigh \gls{pdf} is denoted as $h_{\text{NLOS},n^{\prime}}$, alongside path loss $l_{\text{NLOS},n^{\prime}}$ and shadowing $\zeta_{\text{NLOS},n^{\prime}}$ with respective \gls{NLOS} parameters.
% However, $h_{NLOS,n^{\prime}}$ follows a Rayleigh p.d.f, with the p.d.f of $l_{NLOS,n^{\prime}}$ and $\zeta_{NLOS,n^{\prime}}$ remaining the same as \gls{LOS} channel. 
The parameter $\beta \in (0,1)$ is a smoothing factor which prevents abrupt fluctuations in the channel response caused by transitions between \gls{LOS} and \gls{NLOS} conditions \cite{3gpp2020study}. 
%Furthermore, $\beta$ is parameterized w.r.t the minimum separation distance, $d_{\text{sep}}$.
With the system model in place, we present 
the problem description in the following section.


